A Hybrid Nodal-Staggered Pseudo-Spectral Electromagnetic Particle-In-Cell Method with Finite-Order Centering

Electromagnetic particle-in-cell (PIC) codes are widely used to perform computer simulations of a variety of physical systems, including fusion plasmas, astrophysical plasmas, plasma wakefield particle accelerators, and secondary photon sources driven by ultra-intense lasers. In a PIC code, Maxwell's equations are solved on a grid with a numerical method of choice. This article focuses on pseudo-spectral analytical time-domain (PSATD) algorithms and presents a novel hybrid PSATD PIC scheme that combines the respective advantages of standard nodal and staggered methods. The novelty of the hybrid scheme consists in using finite-order centering of grid quantities between nodal and staggered grids, in order to combine the solution of Maxwell's equations on a staggered grid with the deposition of charges and currents and the gathering of electromagnetic forces on a nodal grid. The correctness and performance of the novel hybrid scheme are assessed by means of numerical tests that employ different classes of PSATD equations in a variety of physical scenarios, ranging from the modeling of electron-positron pair creation in vacuum to the simulation of laser-driven and particle beam-driven plasma wakefield acceleration. It is shown that the novel hybrid scheme offers significant numerical and computational advantages, compared to purely nodal or staggered methods, for all the test cases presented.

==> notes.tex <==
Notes:

### JLV/RL

- Motivations: 
    - [x] also discuss numerical dispersion (in vacuum) with bell curve for nodal
    - [x] advantages gathering fields from nodal grid: no interpolation error between components, especially important for E+VxB with relativistic particles/flows;
    - [x] show some NCI analysis
    - [x] advantages of interpolating from Yee to nodal with high order: ideal is shift in k-space, high-order interpolation is a compromise between locality and accuracy
    - [x] cite paper on PSTD staggered algorithm
    - [x] show EM pulse example to show noise with nodal v. staggered
    - [x] do not mention energy v. momentum conservation

- Section 4: PSATD algorithms on staggered grids
    - [x] emphasize that the algorithms were given in the literature only for nodal grids and were rederived on a Yee grid and summarized here
    - [?] Add all four Maxwell's equations + the continuity equation in sections 4.2 and 4.3 (plus refernce to 4.3 in section 4.4)
    
- Section 5:
    - [x] also show how pure PIC-staggered Galilean is NCI unstable
    - [/] Fig. 2: add vacuum dispersion along x, y and z also
         EZ: not sure now, because of "superluminal" dispersion in the Galilean staggered case, which we do not interpret in any meaningful way yet
    - [/] 5.2: convergence of hybrid (order 8) towards nodal with respect to spectral order
         EZ: closeness of hybrid to nodal does not look better at high spectral order, might be difficult to measure this with our error measure and/or our simulation diagnostics
    - [x] 5.3: try increasing gamma to get test case that is unstable when purely staggered

### EZ

    - [x] Figures in 5.1:
         - colorbar label: replace "B_y" with "B^y"
         - colorbar: maybe put it on the right (a bit more common) and switch with the label "Hybrid Simulations..." that would go on the left?
         - all labels: italic math font (e.g. " label = r'$z$ $[nm]$' ", with the "r" for math notation and square brackets for the units)
         - labels "Hybrid Simulations order 2" etc.: rotate 90 degrees if possible, to save space
         - red annotations: use "B_max" in Figure 5, as "F_max" of Figure 6 (or even better "max(B^y)" and "max(F)")
         - Figure 7: maybe write "max(F)" to save space in the vertical label
         - Figure 7: do we need the zoom inset in linear scale? I'd find the simple log plot clearer to look at and enough for what we want to show
    - [x] Title probably too long (though very self-explanatory right now)
    - [x] Don't know how we are supposed to order the authors of the paper
    - [x] Would be good to double check references as they are cited in the paper (to make sure that it makes sense to cite those references at that point)
    - [x] What do we gain by using the expression "finite-order centering", as opposed to simply "finite-order interpolation"?
    - [x] Check test case description for new test cases (new parameters, etc.)
    - [x] Figures showing stencil extent: label "hybrid" might make people think that a label "staggered" would look different, while the two coincide. Might as well simply use "staggered", as for Figure for vacuum dispersion relation?
    - [x] "Justify" Table 1 (or Figure?) in the text
